Knowledge Distillation for Feature Extraction in Underwater VSLAM

In recent years, learning-based feature detection and matching have outperformed manually-designed methods in in-air cases. However, it is challenging to learn the features in the underwater scenario due to the absence of annotated underwater datasets. This paper proposes a cross-modal knowledge distillation framework for training an underwater feature detection and matching network (UFEN). In particular, we use in-air RGBD data to generate synthetic underwater images based on a physical underwater imaging formation model and employ these as the medium to distil knowledge from a teacher model SuperPoint pretrained on in-air images. We embed UFEN into the ORB-SLAM3 framework to replace the ORB feature by introducing an additional binarization layer. To test the effectiveness of our method, we built a new underwater dataset with groundtruth measurements named EASI (https://github.com/Jinghe-mel/UFEN-SLAM), recorded in an indoor water tank for different turbidity levels. The experimental results on the existing dataset and our new dataset demonstrate the effectiveness of our method.

==> 2_Background/Back.tex <==
\section{Related works}
The focus of our work is to improve the VSLAM performance in a turbid and low-visibility underwater scene. This section covers the four main domains, underwater image formation physical model,  knowledge distillation, visual SLAM and learning local Features, which are involved in our work.

\subsection{Underwater Image Formation Physical Model}
The underwater image formation physical model is the basis of synthetic underwater images and underwater image restoration. Light reflected from the surface of underwater objects attenuates and is absorbed and causes image degradation. In the meantime, the tiny particles in water can lead to backscattering and veiling appearance in the images.

The attenuation and backscattering in underwater imaging are related to the distance from the observed objects to the camera. The commonly used physical underwater imaging model is extracted from the atmospheric scattering model \cite{r1}. In the real physical world, underwater imaging differs from that of atmospheric. The simplified underwater imaging physical model is proposed in \cite{r2}, that is:

\begin{equation}
    U_{\lambda}(x) =  I_{\lambda}(x) \cdot T_{\lambda}(x) + \frac{b(\lambda)E(d, \lambda)}{\beta(\lambda)} \cdot (1 - T_{\lambda}(x))
    \label{equ:1}
\end{equation}

$x$ is the pixel coordinate on the image. The intensity values of x on the captured underwater image is $U_{\lambda}(x)$, on the clear restorage image is $I_{\lambda}(x)$. $T_{\lambda}(x)$ is the medium energy ratio, the attenuation decay term. $B_{\lambda}(x)$ is explained as homogeneous background light. The value of $T_{\lambda}(x)$ is a function of the RGB wavelength $\lambda$ and the distance to the camera $d(x)$. Therefore, that can be expressed as:

\begin{equation}
    T_{\lambda}(x) =  10^{-{\beta}_{\lambda}d(x)} = \frac{E_{\lambda}(x, d(x))}{E_{\lambda}(x, 0)} = N_{\lambda}(d(x))
\end{equation}
$E_{\lambda}(x, 0)$ is the energy of light before the transmission. $E_{\lambda}(x, d(x))$ is the energy after the transmission of a distance $d(x)$. ${\beta}_{\lambda}$ is the attenuation coefficient, which depends on the wavelength of the colour channel. Finally, $N_{\lambda}$ is the normalized residual energy associated with the unit of distance and the wavelength of the light.

Jerlov water types \cite{r3} are the measurements of different attenuation coefficients ${\beta}_{\lambda}$ for different underwater scenarios. It consists of ten water types, including five coastal water types and five open ocean water types. This diversity of water types makes it possible to synthesise underwater images. Authors in \cite{r4},\cite{r5} use these different water types to generate the synthetic underwater datasets to train the image restoration network. However, the assignment of $B_{\lambda}(x)$ is uncertain. It is related to the background light and unevenly distributed in the scene. They used random numbers in a specific range to simulate the underwater environment, but they had to deal with image oversaturation and the discrepancy to the realistic scenarios. 

A revised model is proposed in \cite{r6}, in which the direct and backscattered terms are related to the different coefficients. Moreover, it involves other independent coefficients except for the property coefficients of the water. The revised model is as follows:

\begin{equation}
     U_{\lambda}(x) = I_{\lambda}(x) e^{-\beta_c^D (\textbf{v}_D) \cdot d(x)} + B_c^\infty(1 -  e^{-\beta_c^B (\textbf{v}_B) \cdot d(x)})
    \label{equ:sea_thru}
\end{equation}

This model follows the same logic as Equation \ref{equ:1}. However, it introduces the attenuation terms $\beta_c^D$ and $\beta_c^B$ are two different coefficients and depend on the coefficient vector $\textbf{v}_D$ and $\textbf{v}_B$. Meanwhile, the background light $B_c^\infty$ is assumed to be uniform. The imaging is related to the distance $d(x)$ to the camera. Sea-thru \cite{r7} based on this revised model uses RGB-D dataset to estimate the unknown coefficients and veiling light to restore the authentic attenuated underwater images. 

\subsection{Knowledge Distillation}
Knowledge distillation (KD) was first proposed in \cite{kd1}. Its purpose is to distil the knowledge from an extensive neural network into a relatively small network. It compresses the network to enable an approximate performance in a lighter structure and improves efficiency. There are various types of knowledge in distillation, classified as response-based, feature-based, and relation-based. Response-based knowledge focuses only on the outputs of the teacher model's last layer, while feature-based knowledge uses information from the intermediate layers. Finally, relation-based knowledge is the distillation based on the relationship between layers and samples \cite{kd2}. However, the function of knowledge distillation is not only limited to the compression of the network but also can transfer the knowledge between different data modalities. Sometimes supervision data or labels are little or unavailable for some modalities. The KD strategy Cross-Modal Distillation in \cite{kd3} proposes to transfer knowledge from a rich labelled modality as supervision to an unlabeled paired modality.

Our work utilises cross-modal distillation and transfers the knowledge from the in-air images to the synthetic underwater images. The detected feature points on the in-air images are the labelled supervision data. In contrast, the synthetic underwater images for which it is challenging to obtain supervision labels are the unlabeled modalities.

\subsection{Underwater Visual SLAM}
The framework of visual SLAM consists of two parts: the front and the back end. The front end is also named Visual Odometry (VO), which accepts the perceived measurements and performs feature extraction and data association. The back end is a non-linear optimisation to remove the accumulated noise in SLAM and perform the global map estimation \cite{kd4}. Depending on how the constraints are extracted at the front end, they can be divided into feature-based methods and direct methods \cite{kd5}. Feature-based SLAM is the use of sparse feature points to construct 3D landmarks in space, and the direct methods estimate the motion trajectory based on the intensity of pixel values on continuous images.

A popular feature-based method, ORB-SLAM \cite{kd6_2}, \cite{kd6_1}, \cite{kd6}, proposes a VSLAM framework that consists of tracking, mapping, relocalisation, and loop closing. It uses a binary descriptor ORB \cite{kd7} to give the identity of spatial feature points at different distances to achieve a real-time system. It also uses a keyframe-based approach to detect loop closure, thus eliminating the drift that accumulates over time. Some existing works embed the trained neural network into the ORB-SLAM framework to overcome the specific issue \cite{kd8} or improve the VSLAM performance \cite{kd9}. 


\subsection{Learning local Features}
Extracting and matching local features on the image frames is an essential step of some VO and VSLAM \cite{kd6_2}, \cite{kd6_1}, \cite{kd6}. The handcrafted features, such as SIFT \cite{kd10}, ORB \cite{kd7}, can directly find the potential interest feature points on the images based on the raw image data. The use of neural networks to detect feature points and assign descriptors has also been widely studied and has shown promising results \cite{kd11} \cite{kd12} \cite{superpoint}. SuperPoint \cite{superpoint} is a self-supervised solution with a competitive performance on the HPatches dataset \cite{hpatches}. It is firstly trained by the labelled corners of the synthetic shapes. After that, a novel Homographic Adaptation procedure could generate a combined label image from several self-warp labelled images to self-supervision. The last step is the join training to ensure the detected interest points' descriptors could match different image frames and remove the redundant detected feature points. 

Because SuperPoint is initially trained on corner points of the synthetic general shapes, this training makes SuperPoint somewhat general and applicable to different scenarios, tending to focus on corner points in the environment, i.e., on pixels with significant changes in pixel intensity, similar to the principle of FAST \cite{kd13}. We use the pre-trained model provided by the authors in \cite{superpoint} as the teacher model in our work.

